Instance Brownian Bridge as Texts for Open-vocabulary Video Instance Segmentation

Temporally locating objects with arbitrary class texts is the primary pursuit of open-vocabulary Video Instance Segmentation (VIS). Because of the insufficient vocabulary of video data, previous methods leverage image-text pretraining model for recognizing object instances by separately aligning each frame and class texts, ignoring the correlation between frames. As a result, the separation breaks the instance movement context of videos, causing inferior alignment between video and text. To tackle this issue, we propose to link frame-level instance representations as a Brownian Bridge to model instance dynamics and align bridge-level instance representation to class texts for more precisely open-vocabulary VIS (BriVIS). Specifically, we build our system upon a frozen video segmentor to generate frame-level instance queries, and design Temporal Instance Resampler (TIR) to generate queries with temporal context from frame queries. To mold instance queries to follow Brownian bridge and accomplish alignment with class texts, we design Bridge-Text Alignment (BTA) to learn discriminative bridge-level representations of instances via contrastive objectives. Setting MinVIS as the basic video segmentor, BriVIS surpasses the Open-vocabulary SOTA (OV2Seg) by a clear margin. For example, on the challenging large-vocabulary VIS dataset (BURST), BriVIS achieves 7.43 mAP and exhibits 49.49% improvement compared to OV2Seg (4.97 mAP).

==> tab/tir_bta_ablation.tex <==
\begin{table*}
\centering                         % 控制表格居中
\renewcommand{\arraystretch}{1.4}  % 控制行高
\setlength{\tabcolsep}{1.3mm}      % 控制列间距
\footnotesize                      % 控制字体大小
\begin{subtable}[t]{0.49\textwidth}
\caption{TIR}
\begin{tabular}{x{33}x{33}|y{37}y{37}y{37}}
\noalign{\hrule height 1.5pt}
{Inter-frame} & {Intra-frame} & \multicolumn{1}{c}{{mAP$_{a}$}} & \multicolumn{1}{c}{{mAP$_{c}$}} & \multicolumn{1}{c}{{mAP$_{u}$}} \\
\hline
\cmark      &             & 5.82 & 9.44 & 4.92 \\
            & \cmark      & 6.53~\increase{0.71}  & 9.49~\increase{0.05} & 5.78~\increase{0.86} \\
\rowcolor{aliceblue}
\cmark      & \cmark      & \textbf{6.53~\increase{1.61}} & \textbf{9.49~\increase{0.09}} & \textbf{5.78~\increase{1.99}}\\
\noalign{\hrule height 1.5pt}
\end{tabular}
\end{subtable}
\hfill
\begin{subtable}[t]{0.49\textwidth}
\caption{BTA~($\mathbfcal{L}_{bta}$)}
\begin{tabular}{x{20}x{20}x{20}|y{37}y{37}y{37}}
\noalign{\hrule height 1.5pt}
% \hline
$\mathbfcal{L}_{htm}$ Eq.~\ref{eq:htm} & $\mathbfcal{L}_{bc}$ Eq.~\ref{eq:bc} & $\mathbfcal{L}_{btc}$ Eq.~\ref{eq:btc} & \multicolumn{1}{c}{{mAP$_{a}$}} & \multicolumn{1}{c}{{mAP$_{c}$}} & \multicolumn{1}{c}{{mAP$_{u}$}} \\
\hline
       & \cmark & \cmark & 5.82 & 9.44 & 4.92 \\
\hdashline
\cmark &        & \cmark & 6.53~\increase{0.71}  & 9.49~\increase{0.05} & 5.78~\increase{0.86} \\
\rowcolor{aliceblue}
\cmark & \cmark & \cmark & \textbf{7.43~\increase{1.61}} & \textbf{9.53~\increase{0.09}} & \textbf{6.91~\increase{1.99}}\\
\noalign{\hrule height 1.5pt}
\end{tabular}
\end{subtable}
\caption{\textbf{Ablation Study} of (a) TIR sub-modules, i.e., Inter-frame module and Intra-frame module; (b) BTA sub-objectives, i.e., Head-Tail Matching~($\mathbfcal{L}_{htm}$, Equation~\ref{eq:htm}), Bridge Contrastive~($\mathbfcal{L}_{bc}$, Equation~\ref{eq:bc}), and Bridge-Text Contrastive~($\mathbfcal{L}_{btc}$, Equation~\ref{eq:btc}). We follow the evaluation strategy and settings of Table~\ref{tab:main_abl}.}
\label{tab:bta_abl}
\end{table*}

